On the Smart Coordination of Flexibility Scheduling in Multi-carrier Integrated Energy Systems

Coordinating the interactions between flexibility assets in multi-carrier integrated energy systems (MIES) can lead to an efficient integration of variable renewable energy resources, and a cost-efficient energy transition. However, the proliferation of flexibility assets and their participation in active demand response increases the complexity of coordinating these interactions. This paper introduces different approaches to model the coordination of flexibility scheduling in MIES. We propose a market auction-inspired model coupling approach to address the challenges of preserving the autonomy and privacy of flexibility providers, and the issue of scalability. We benchmark our approach against co-optimization and an iterative price-response method by conducting experiments with varying problem sizes and computing infrastructure. We show that our approach scales well and is suitable for modeling flexibility in large-scale energy systems in a more realistic way. From an optimality standpoint, the flexibility dispatch schedules and electricity prices are ``near-optimal". Our methodology is implemented as a new open-source software, which offers several practical applications. For example, flexibility providers and network operators can couple their models to simulate the interaction between their systems without disclosing confidential information; policy regulators can use it to investigate new market design and regulations to optimize the utilization of flexibility in MIES.

==> figures/src/MIES.tex <==
\section{Multi-carrier integrated energy system}

\begin{figure*}[h] % ADMM-model interactions
\begin{tikzpicture}[scale=0.95]

    % ########### Electric bus components #########
    % Draw electric bus
    \path[draw, line width=0.7mm, name path=eBusLine] (-0.8, -2) -- (10.7, -2);
    \node[align=center, font=\scriptsize] at (0.2, -1.5) {Electric \\ bus};

    % Draw generator (circle with a tilde inside)
    \draw (2,-0.8) circle (0.4cm); % Draw the circle
    \node at (2,-0.8) {$\sim$}; % Place the tilde symbol at the center of the circle
    
    % Draw rectangle with dashed lines
    \node[draw=black, dashed, rectangle, minimum width=2.5cm, minimum height=1.5cm, align=center, font=\scriptsize] (Generatoragentrboundary) at (2.5, -1) {};
    
    % Draw a vertical line connecting the electric bus to the electric generator
    \draw[->, >=latex, line width=0.2mm] (2, -1.2) -- (2, -2);

    % Traditional electric load triangle
    \coordinate (A) at (5, -0.5);  % top vertex
    \coordinate (B) at (4.5, -1.0);     % bottom-left vertex
    \coordinate (C) at (5.5, -1.0);     % bottom-right vertex
    % Draw the triangle
    \draw (A) -- (B) -- (C) -- cycle;

    % Draw a vertical line connecting the electric bus to the electric load
    \draw[-, line width=0.1mm] (5, -2) -- (5, -1);


    % Electric storage rectangle, name, and connecting arrow
    \node[draw, rectangle, minimum width=1.3cm, minimum height=0.6cm, align=center, font=\scriptsize] (electricstoragerect) at (8.5, -0.7) {};
    \node[rectangle, minimum width=0.5cm, minimum height=1cm, align=center, font=\scriptsize] (storage) at (8.5, -0.7) {Battery};
    % Draw double head arrow connecting electric storage to electric bus
    \draw[<->, >=latex, line width=0.2mm] (8.5, -2) -- (8.5, -1);

    % Draw rectangle with dashed lines
    \node[draw=black, dashed, rectangle, minimum width=2cm, minimum height=1.5cm, align=center, font=\scriptsize] (Generatoragentrboundary) at (8.5, -1) {};

    % % Interconnector line
    % \draw[<->, >=latex, line width=0.2mm] (8.5, -0.9) -- (8.5, -2);
    % \node[rectangle, minimum width=0.5cm, minimum height=1cm, align=center, font=\scriptsize] (gridconncetion) at (8.8, -0.7) {Grid connection};
    
    %%%%%% Name electric bus components
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize,] (generators) at (2.9, -1.5) {Generator};

    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize,] (eload) at (5.9, -1.5) {Traditional \\ electric load};

    % ############# Heat bus components #########
     % Draw heat bus
    \path[draw, line width=0.7mm, name path=HeatBusLine] (-0.2, -4) -- (3.4, -4);
    \node[align=center, font=\scriptsize, text=black] at (0.5, -3.5) {Heat \\ bus};

    % Draw rectangle with dashed lines
     \node[draw=black, dashed, rectangle, minimum width=4.45cm, minimum height=3.8cm, align=center, font=\scriptsize] (Heatprosumerboundary) at (1.55, -4.2) {};
    
    % Heat load
    \coordinate (H) at (0.7, -5.9);   % bottom vertex
    \coordinate (I) at (0.3, -5.4); % top-left vertex
    \coordinate (J) at (1.1, -5.4); % top-right vertex
    % Draw the triangle
    \draw (H) -- (I) -- (J) -- cycle;
    % Draw a vertical line connecting heat bus to heat load
    \draw[-, line width=0.1mm] (0.7, -4) -- (0.7, -5.4);

    % Draw Solarthermal generation circle 
    \draw (3.2,-5.4) circle (0.4cm); % Draw the circle
    % Draw a vertical line connecting heat bus to Solarthermal source
    \draw[->, >=latex, line width=0.2mm] (3.2, -5) -- (3.2, -4);

    %%%%%% Name heat bus components
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize,] (thermalgeneration) at (2.7, -6) {Solarthermal};

    % Heat storage rectangle, name, and connecting arrow
    \node[draw, rectangle, minimum width=1.1cm, minimum height=0.6cm, align=center, font=\scriptsize,] (heatstoragerect) at (2.1, -5.4) {};
    \node[rectangle, minimum width=0.5cm, minimum height=1cm, align=center, font=\scriptsize] (thermalstorage) at (2.1, -5.4) {Storage};
    % Draw double head arrow connecting heat storage to heat bus
    \draw[<->,  >=latex, line width=0.2mm] (2.1, -5.1) -- (2.1, -4);

     % Draw Hydrogen boiler
    \draw[-,  >=latex, line width=0.2mm] (3.7, -6.3) -- (3.7, -2.5);
    \draw[-,  >=latex, line width=0.2mm] (2.7, -2.5) -- (3.7, -2.5);
    \draw[<-,  >=latex, line width=0.2mm] (2.7, -4) -- (2.7, -2.5);
    \node[rectangle, minimum width=1cm, minimum height=1cm, rotate=90, align=center, font=\scriptsize,] (thermalgeneration) at (2.4, -3.2) {H2-boiler};

    % ########### Hydrogen bus components #########
    % Draw hydrogen bus
    \path[draw, line width=0.7mm, name path=HyrogenBusLine] (4.5, -4) -- (7.2, -4);
    \node[align=center, font=\scriptsize] at (5.2, -3.5) {Hydrogen \\ bus};

    % Draw rectangle with dashed lines
     \node[draw=black, dashed, rectangle, minimum width=2.85cm, minimum height=3.8cm, align=center, font=\scriptsize] (Hydrogenprosumerboundary) at (5.9, -4.2) {};
    
    % Hydrogen load
    \coordinate (O) at (7.3 - 1.8, -5.9);     % bottom vertex
    \coordinate (P) at (6.8 - 1.8, -5.4); % top-left vertex
    \coordinate (Q) at (7.8 - 1.8, -5.4); % top-right vertex
    % Draw the triangle
    \draw (O) -- (P) -- (Q) -- cycle;

    % Draw a vertical line connecting hydrogen bus to hydrogen load
    \draw[-, line width=0.1mm] (5.5, -4) -- (5.5, -5.4);
    
    %%%%%% Name hydrogen bus components
    % Hydrogen store rectangle, name, and connecting arrow
    % \node[draw, rectangle, minimum width=1.1cm, minimum height=0.6cm, align=center, font=\scriptsize,] (hydrogenstoragerect) at (4.8, -5.5) {};
    % \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize,] (hydrogenstorage) at (4.8, -5.5) {Store};
    
    % Draw single-head arrow connecting hydrogen store to hydrogen bus
    \draw[->,  >=latex, line width=0.2mm] (4.9, -6.3) -- (4.9, -4);
    
    % Hydrogen storage rectangle, name, and connecting arrow
    \node[draw, rectangle, minimum width=1.1cm, minimum height=0.6cm, align=center, font=\scriptsize,] (hydrogenstoragerect) at (6.7, -5.5) {};
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize,] (hydrogenstorage) at (6.7, -5.5) {Storage};
    % Draw double head arrow connecting heat storage to heat bus
    \draw[<->,  >=latex, line width=0.2mm] (6.7, -5.2) -- (6.7, -4);
    
    % ######### Transport bus components #########
    % Draw Transport bus
    \path[draw, line width=0.7mm, name path=TransportBusLine] (8.1, -4) -- (10.5, -4);
    \node[align=center, font=\scriptsize] at (8.63, -3.5) {Transport \\ bus};

    % Draw rectangle with dashed lines
     \node[draw=black, dashed, rectangle, minimum width=2.5cm, minimum height=3.8cm, align=center, font=\scriptsize] (Transportprosumerboundary) at (9.2, -4.2) {};
    
   % Transport load
    \coordinate (R) at (10.5 - 2, -5.9); % bottom vertex
    \coordinate (S) at (10 - 2, -5.4); % top-left vertex
    \coordinate (T) at (11 - 2, -5.4); % top-right vertex
    % Draw the triangle
    \draw (R) -- (S) -- (T) -- cycle;

     % Draw a vertical line connecting transport bus to EV battery storage
    \draw[-, line width=0.1mm] (8.5, -4) -- (8.5, -5.4);

     %%%%%% Name transport bus components
    % Hydrogen storage rectangle, name, and connecting arrow
    \node[draw, rectangle, minimum width=1.1cm, minimum height=0.6cm, align=center, font=\scriptsize,] (evbatteryrect) at (9.7, -5.5) {};
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize,] (hydrogenstorage) at (9.7, -5.5) {Battery};
    % Draw double head arrow connecting heat storage to heat bus
    \draw[<->,  >=latex, line width=0.2mm] (9.7, -5.2) -- (9.7, -4);

    % ######### Methane/biomass bus components #########
    % Draw Methane and biomass bus
    \path[draw, line width=0.7mm, name path=MethaneBusLine] (-0.5, -6.3) -- (0.7, -6.3);
    \node[align=center, font=\scriptsize] at (-0.3, -7) {Methane \\ source};
    \path[draw, line width=0.7mm, name path=BiomassBusLine] (0.9, -6.3) -- (2, -6.3);
    \node[align=center, font=\scriptsize] at (2.1, -7) {Biomass \\ source};

    %%%%%% Name methane bus components
     % Heat storage rectangle, name, and connecting arrow
    % \node[draw, rectangle, minimum width=1.1cm, minimum height=0.6cm, align=center, font=\scriptsize,] (methanestorerect) at (0.6, -7.5) {};
    % \node[rectangle, minimum width=0.5cm, minimum height=1cm, align=center, font=\scriptsize] (methanestore) at (0.6, -7.5) {Store};

    % Draw arrow for external methane source
    \draw[->,  >=latex, line width=0.2mm] (0.4, -6.8) -- (0.4, -6.3);
    \draw[dashed, >=latex, line width=0.2mm] (0.4, -7.5) -- (0.4, -6.8);

    % Draw arrow for external biomass source
    \draw[->,  >=latex, line width=0.2mm] (1.4, -6.8) -- (1.4, -6.3);
    \draw[dashed, >=latex, line width=0.2mm] (1.4, -7.5) -- (1.4, -6.8);

    % ######### External Hydrogen source bus #########
    \path[draw, line width=0.7mm, name path=ExternalH2SourceBusLine] (3.3, -6.3) -- (5.8, -6.3);
    \node[align=center, font=\scriptsize] at (5, -7) {External \\ H2 source};
    \draw[->,  >=latex, line width=0.2mm] (4.2, -6.8) -- (4.2, -6.3);
    \draw[dashed, >=latex, line width=0.2mm] (4.2, -7.5) -- (4.2, -6.8);

    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (H2-transport) at (5.2, -5.2) {H2 pipeline};

    
    % ########## Connect buses with p2x techs ############
    % Draw vertical arrows connecting the electric bus and heat bus
    \draw[->, >=latex, line width=0.2mm] (1.2, -2) -- (1.2, -4); % Heatpump
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (heatpump) at (2.15, -3.05) {Heat pump; \\ E-boiler};
    % \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (eboiler) at (2.25, -3) {};

    % Draw vertical arrows connecting the electric bus to hydrogen bus
    \draw[->, >=latex, line width=0.2mm] (6, -2) -- (6, -4);  % Electrolyzer
    \draw[<-, >=latex, line width=0.2mm] (6.8, -2) -- (6.8, -4);  % Fuel cell
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (electrolyzer) at (6.75, -3) {Electrolyzer};
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (fuelcell) at (7.6, -3) {Fuel cell};

     % Draw vertical arrows connecting the electric bus to transport bus
    \draw[->, >=latex, line width=0.2mm] (9.4, -2) -- (9.4, -4);  % EV-charge
    \draw[<-, >=latex, line width=0.2mm] (10, -2) -- (10, -4);  % EV-discharge
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (charge) at (10.2, -3) {EV-charge};
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (discharge) at (10.8, -3) {EV-discharge};

    % Draw vertical arrows connecting the methane bus to electric bus (gasgenerators)
    \draw[<-, >=latex, line width=0.2mm] (-0.35, -2) -- (-0.35, -6.27); % CHP; Gas generators
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (gasgenerator) at (-0.01, -4.2) {CHP};

    % Draw vertical arrows connecting the heat bus to methane bus
    \draw[<-, >=latex, line width=0.2mm] (0.2, -4) -- (0.2, -6.27); % CHP; boiler
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (chpgasboiler) at (0.5, -5.2) {CHP; Boiler};

    % Draw vertical arrows connecting the heat bus to biomass bus
    \draw[<-, >=latex, line width=0.2mm] (1.4, -4) -- (1.4, -6.27); % biomass boiler
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (biomassboiler) at (1.7, -4.8) {Boiler};
    
\end{tikzpicture}
\end{figure*}

==> figures/src/admm.tex <==
\section{ADMM-inspired solution method}

\begin{figure*}[h] % ADMM-model interactions
\begin{tikzpicture}[scale=0.95]
    % Draw an invisible rectangle to write iteration k, k+1, k+n
    \node[rectangle, minimum width=1.8cm, minimum height=1cm, align=center, font=\scriptsize] (iterrect1) at (2,3) {Iteration $k$};
    \node[rectangle, minimum width=1.8cm, minimum height=1cm, align=center, font=\scriptsize] (iterrect2) at (11.5,3) {Iteration $k+1$};
    
    % \node[rectangle, minimum width=1.8cm, minimum height=1cm, align=center, font=\scriptsize] (iterrectn) at (16.5,3) {Iteration $k+n$};

    % Put the price update equation in a rectangle with invisible outlines
    \node[rectangle, minimum width=5cm, minimum height=1cm, align=center, font=\scriptsize] (invisiblerect1) at (6.8, -1.0) {
        \begin{varwidth}{\linewidth}
       \[
            \lambda^{k} = \lambda^{k-1} - \rho \cdot I^{k}
        \]
        \end{varwidth}
    };

    % Put the text "price update for next iteration in an invisible rectangle"
    \node[rectangle, minimum width=1.8cm, minimum height=1cm, align=center, font=\scriptsize] (invisiblerect2) at (6.7, -0.3) {Price update for iteration $k+1$};
    
    % Draw the three rounded edge rectangles aligned at the top (Left)
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect1) at (0,2) {Generator \\ agent 1};
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect2) at (1.8,2) {Generator \\ agent 2};
    % invisible rectangle for the ... sign for generators 1 ... n
    \node[rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (lefttopinvisiblerect) at (2.9,2) {...};
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect3) at (4,2) {Generator \\ agent n};
    
    % Draw a squared edge rectangle below the previous ones (Left)
    \node[draw, rectangle, minimum width=4.5cm, minimum height=1cm, align=center, font=\scriptsize] (leftmidrect) at (2, -0.6) {Coordinator agent \\
        \begin{varwidth}{\linewidth}
        \[
            I^{k} = \frac{1}{\left|{N}\right| + 1} \sum_{i, j} ({g^{k}_{i}} + {p^{k}_{j}})
        \]
        \end{varwidth}
    };
    
    % Draw three rounded edge rectangles aligned at the bottom (Left)
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect4) at (0, -3.2) {Prosumer \\ agent 1};
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect5) at (1.8, -3.2) {Prosumer \\ agent 2};
    % invisible rectangle for the ... sign for prosumers 1 ... n
    \node[rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftbottominvisiblerect) at (2.9,-3.2) {...};
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect6) at (4, -3.2) {Prosumer \\ agent n};
    
    % Draw the three rounded edge rectangles aligned at the top (Right)
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (rightrect1) at (9.6,2) {Generator \\ agent 1};
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (rightrect2) at (11.4,2) {Generator \\ agent 2};
    % invisible rectangle for the ... sign for generators 1 ... n
    \node[rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (righttopinvisiblerect) at (12.5,2) {...};
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (rightrect3) at (13.6,2) {Generator \\ agent n};
    
    % Draw the squared edge rectangle below the previous ones (Right)
    \node[draw, rectangle, minimum width=4.5cm, minimum height=1cm, align=center, font=\scriptsize] (rightmidrect) at (11.6, -0.6) {Coordinator agent \\
        \begin{varwidth}{\linewidth}
        \[
            I^{k+1} = \frac{1}{\left|{N}\right| + 1} \sum_{i, j} ({g^{k+1}_{i}} + {p^{k+1}_{j}})
        \]
        \end{varwidth}
    };
    
    % Draw three rounded edge rectangles aligned at the bottom (Right)
    \node[draw, rectangle, rounded corners,  minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (rightrect4) at (9.6, -3.2) {Prosumer \\ agent 1};
    \node[draw, rectangle, rounded corners,  minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (rightrect5) at (11.4, -3.2) {Prosumer \\ agent 2};
    % invisible rectangle for the ... sign for prosumers 1 ... n
    \node[rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (rightbottominvisiblerect) at (12.5,-3.2) {...};
    \node[draw, rectangle, rounded corners,  minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (rightrect6) at (13.6, -3.2) {Prosumer \\ agent n};

    % Put the text "{...}" inside it
    % \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (invisiblerectbesideinvisibleone) at (16.5, -0.6) {...};
    
    % Arrows connecting rounded edge rectangles (left) to the left middle rectangle (leftmidrect)

    % Arrows connecting top rectangles (left) to leftmidrect
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect1.south) -- ++(0, -0.3) -- ([xshift=-0.1cm]leftmidrect.north -| leftrect1.south);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect1.south) -- ++(0, -0.3) -- ([xshift=0.1cm] leftmidrect.north -| leftrect1.south);
    
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect2.south) -- ++(0, -0.3) -- ([xshift=-0.1cm] leftmidrect.north -| leftrect2.south);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect2.south) -- ++(0, -0.3) -- ([xshift=0.1cm] leftmidrect.north -| leftrect2.south);
    
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect3.south) -- ++(0, -0.3) -- ([xshift=-0.1cm] leftmidrect.north -| leftrect3.south);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect3.south) -- ++(0, -0.3) -- ([xshift=0.1cm] leftmidrect.north -| leftrect3.south);

    
    % Arrows connecting bottom rectangles (left) to leftmidrect
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect4.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] leftmidrect.south -| leftrect4.north);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect4.north) -- ++(0, 0.3) -- ([xshift=0.1cm] leftmidrect.south -| leftrect4.north);
    
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect5.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] leftmidrect.south -| leftrect5.north);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect5.north) -- ++(0, 0.3) -- ([xshift=0.1cm] leftmidrect.south -| leftrect5.north);
    
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect6.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] leftmidrect.south -| leftrect6.north);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect6.north) -- ++(0, 0.3) -- ([xshift=0.1cm] leftmidrect.south -| leftrect6.north);
    
     % Arrows connecting rounded edge rectangles (right) to the right middle rectangle (rightmidrect)

    % Arrows connecting top rectangles (right) to rightmidrect
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] rightrect1.south) -- ++(0, -0.3) -- ([xshift=-0.1cm] rightmidrect.north -| rightrect1.south);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] rightrect1.south) -- ++(0, -0.3) -- ([xshift=0.1cm] rightmidrect.north -| rightrect1.south);
    
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm]  rightrect2.south) -- ++(0, -0.3) -- ([xshift=-0.1cm] rightmidrect.north -| rightrect2.south);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm]  rightrect2.south) -- ++(0, -0.3) -- ([xshift=0.1cm] rightmidrect.north -| rightrect2.south);
    
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] rightrect3.south) -- ++(0, -0.3) -- ([xshift=-0.1cm] rightmidrect.north -| rightrect3.south);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] rightrect3.south) -- ++(0, -0.3) -- ([xshift=0.1cm] rightmidrect.north -| rightrect3.south);
    
    % Arrows connecting bottom rectangles (right) to rightmidrect
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] rightrect4.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] rightmidrect.south -| rightrect4.north);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] rightrect4.north) -- ++(0, 0.3) -- ([xshift=0.1cm] rightmidrect.south -| rightrect4.north);
    
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] rightrect5.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] rightmidrect.south -| rightrect5.north);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] rightrect5.north) -- ++(0, 0.3) -- ([xshift=0.1cm] rightmidrect.south -| rightrect5.north);
    
    \draw[<-, >=latex, line width=0.1mm] ([xshift=-0.1cm] rightrect6.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] rightmidrect.south -| rightrect6.north);
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.1cm] rightrect6.north) -- ++(0, 0.3) -- ([xshift=0.1cm] rightmidrect.south -| rightrect6.north);

    % Long horizontal arrow connecting the two squared edge middle rectangles
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.05cm] leftmidrect.east) -- ([xshift=-0.05cm] rightmidrect.west);

    % Add texts beside vertical arrows (left side of figure)
    % Generator agent 1
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftHeatOperator) at (-0.45,1) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftHeatOperator) at (-0.45,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightHeatOperator) at (0.4,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            g^{k}_{1}
        \]
    \end{varwidth}
    };
    % Generator agent 2
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftEVOperator) at (1.35,1) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftHeatOperator) at (1.35,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightEVOperator) at (2.2,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            g^{k}_{2}
        \]
    \end{varwidth}
    };
     % Generator agent n
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftBEESOperator) at (3.55,1) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftHeatOperator) at (3.55,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightBEESOperator) at (4.4,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            g^{k}_{n}
        \]
    \end{varwidth}
    };
    % Prosumer agent 1
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftElectrolyzer) at (-0.45,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftElectrolyzer) at (-0.45,-2.2) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightElectrolyzer) at (0.4,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            p^{k}_{1}
        \]
    \end{varwidth}
    };
    % Prosumer agent 2
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftTradLoad) at (1.35,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftTradLoad) at (1.35,-2.2) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightTradLoad) at (2.2,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            p^{k}_{2}
        \]
    \end{varwidth}
    };
    % Prosumer agent n
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftGeneration) at (3.55,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftGeneration) at (3.55,-2.2) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k-1}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightGeneration) at (4.4,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            p^{k}_{n}
        \]
    \end{varwidth}
    };


    % Add texts beside vertical arrows (right side of figure)
    % Generator 1 iteration k+1
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftHeatOperator) at (9.3,1) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftHeatOperator) at (9.3,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightHeatOperator) at (10.2,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            g^{k+1}_{1}
        \]
    \end{varwidth}
    };
    % Generator 2 iteration k+1
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftEVOperator) at (11.1,1) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftEVOperator) at (11.1,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightEVOperator) at (12,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            g^{k+1}_{2}
        \]
    \end{varwidth}
    };
    % Generator n iteration k+1
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftBEESOperator) at (13.3,1) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftBEESOperator) at (13.3,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightBEESOperator) at (14.2,0.5) {
    \begin{varwidth}{\linewidth}
       \[
            g^{k+1}_{n}
        \]
    \end{varwidth}
    };
    % Prosumer 1 iteration k+1
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftElectrolyzer) at (9.3,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftElectrolyzer) at (9.3,-2.2) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightElectrolyzer) at (10.2,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            p^{k+1}_{1}
        \]
    \end{varwidth}
    };
    % Prosumer 2 iteration k+1
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftTradLoad) at (11.1,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftTradLoad) at (11.1,-2.2) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightTradLoad) at (12,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            p^{k+1}_{2}
        \]
    \end{varwidth}
    };
    % Prosumer n iteration k+1
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftGeneration) at (13.3,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            I^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftGeneration) at (13.3,-2.2) {
    \begin{varwidth}{\linewidth}
       \[
            \lambda^{k}
        \]
    \end{varwidth}
    };
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightGeneration) at (14.2,-1.7) {
    \begin{varwidth}{\linewidth}
       \[
            p^{k+1}_{n}
        \]
    \end{varwidth}
    };

    % ====================== Arrows at start and end of figure ===================
    % Draw the invisible squared edge righrihtrectangle (RightRight)
    \node[rectangle, minimum width=5cm, minimum height=1cm, align=center, font=\scriptsize] (rightrightmidrect) at (17.5, -0.6) {};
    % Long horizontal arrow connecting the right squared edge middle rectangle to unknown one
    \draw[->, >=latex, line width=0.1mm] ([xshift=0.05cm] rightmidrect.east) -- ([xshift=-0.05cm] rightrightmidrect.west);
    \node[rectangle, minimum width=1.8cm, minimum height=1cm, align=center, font=\scriptsize] (iterrectbetweenk+1andn) at (15.2,-0.6) {...};
    
    % Long horizontal arrow connecting unknown to the left squared edge middle rectangle
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftleftmidrect) at (-1.8, -0.6) {};
    \draw[->, >=latex, line width=0.1mm] (leftleftmidrect.east) -- ([xshift=-0.05cm] leftmidrect.west);
     \node[rectangle, minimum width=1.8cm, minimum height=1cm, align=center, font=\scriptsize] (iterrectbetweenk-1andk) at (-1.7,-0.6) {...};
    % ==========================================================================
    
\end{tikzpicture}
\end{figure*}

==> figures/src/co_optim.tex <==
\section{Co-optimization problem}

\begin{figure*}[h]
 % \centering
\begin{tikzpicture}[scale=0.95]
    % Draw co-optimization main frame
    % \node[draw, rectangle, rounded corners, minimum width=12cm, minimum height=8cm, font=\scriptsize, dash pattern=on 5pt off 3pt] (mainrectframe) at (3.5,-0.6) {};

    % Draw the three rounded edge rectangles aligned at the top (Left)
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect1) at (-0.5 + 0.5,3) {Generator agent 1};
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect2) at (2 + 2,3) {Generator agent 2};
    % invisible rectangle for the ... sign for generators 1 ... n
    \node[rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (lefttopinvisiblerect) at (3.5 + 3,2.95) {...};
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect3) at (5 + 4,3) {Generator agent n};
    
    % Draw a squared edge rectangle below the previous ones (Left)
    \node[draw, rectangle, minimum width=10cm, minimum height=2cm, align=center, font=\scriptsize] (leftmidrect) at (4.5, -0.6) {Central agent \\
        \begin{varwidth}{\linewidth}
        \[
            \textstyle  \underset{g_{1} ... g_{n}, p_{1} ... p_{n}}\max \prod_{global} \big( \displaystyle g_{1} ... g_{n}, p_{1} ... p_{n}, \phi \big)
        \]
        \end{varwidth}
        \\
         \begin{varwidth}{\linewidth}
            \[
              \text{s.t.} \quad g_{1} \in G_{1}, g_{2} \in G_{2}, ..., g_{n} \in G_{n}
            \]
        \end{varwidth}
        \\
         \begin{varwidth}{\linewidth}
            \[
               \quad \quad  p_{1} \in P_{1}, p_{2} \in P_{2}, ..., p_{n} \in P_{n}
            \]
        \end{varwidth}
        \\
        \begin{varwidth}{\linewidth}
            \[
               \quad \qquad  \sum^{N_{G}}_{i=1} {g_{i}} + \sum^{N_{P}}_{j=1} {p_{j}} = 0: \quad \quad \lambda
            \]
        \end{varwidth}
    };
    
    % Draw three rounded edge rectangles aligned at the bottom (Left)
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect4) at (-0.5 + 0.5, -4.2) {Prosumer agent 1};
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect5) at (2 + 2, -4.2) {Prosumer agent 2};
    % invisible rectangle for the ... sign for prosumers 1 ... n
    \node[rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftbottominvisiblerect) at (3.5 + 3,-4.2) {...};
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftrect6) at (5 + 4, -4.2) {Prosumer agent n};
    
    
    % Arrows connecting rounded edge rectangles (left) to the left middle rectangle (leftmidrect)

    % Arrows connecting top rectangles (left) to leftmidrect
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect1.south) -- ++(0, -0.3) -- ([xshift=-0.1cm]leftmidrect.north -| leftrect1.south);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect1.south) -- ++(0, -0.3) -- ([xshift=0.1cm] leftmidrect.north -| leftrect1.south);
    
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect2.south) -- ++(0, -0.3) -- ([xshift=-0.1cm] leftmidrect.north -| leftrect2.south);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect2.south) -- ++(0, -0.3) -- ([xshift=0.1cm] leftmidrect.north -| leftrect2.south);
    
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect3.south) -- ++(0, -0.3) -- ([xshift=-0.1cm] leftmidrect.north -| leftrect3.south);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect3.south) -- ++(0, -0.3) -- ([xshift=0.1cm] leftmidrect.north -| leftrect3.south);

    
    % Arrows connecting bottom rectangles (left) to leftmidrect
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect4.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] leftmidrect.south -| leftrect4.north);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect4.north) -- ++(0, 0.3) -- ([xshift=0.1cm] leftmidrect.south -| leftrect4.north);
    
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect5.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] leftmidrect.south -| leftrect5.north);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect5.north) -- ++(0, 0.3) -- ([xshift=0.1cm] leftmidrect.south -| leftrect5.north);
    
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect6.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] leftmidrect.south -| leftrect6.north);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect6.north) -- ++(0, 0.3) -- ([xshift=0.1cm] leftmidrect.south -| leftrect6.north);

    
    % Add texts beside vertical arrows (left side of figure)
    % Generator agent 1
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftHeatOperator) at (-1.4,1.35) {complete \\ information of $G_{1}$};
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightHeatOperator) at (0.15 + 0.5,2.2) {
    \begin{varwidth}{\linewidth}
       \[
            (\lambda, g_{1})
        \]
    \end{varwidth}
    };
    % Generator agent 2
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftEVOperator) at (1.05 + 1.5,1.35) {complete \\ information of $G_{2}$};
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightEVOperator) at (2.65 + 2, 2.2) {
    \begin{varwidth}{\linewidth}
       \[
             (\lambda, g_{2})
        \]
    \end{varwidth}
    };
     % Generator agent n
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftBEESOperator) at (4 + 3.5,1.35) {complete \\ information of $G_{n}$};
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightBEESOperator) at (5.7 + 4,2.2) {
    \begin{varwidth}{\linewidth}
       \[
            (\lambda, g_{n})
        \]
    \end{varwidth}
    };
    % Prosumer agent 1
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftElectrolyzer) at (-1.4,-2.55) {complete \\ information of $P_{1}$};
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightElectrolyzer) at (0.15 + 0.5,-3.4) {
    \begin{varwidth}{\linewidth}
       \[
            (\lambda, p_{1})
        \]
    \end{varwidth}
    };
    % Prosumer agent 2
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftTradLoad) at (1.1 + 1.5,-2.55) {complete \\ information of $P_{2}$};
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightTradLoad) at (2.65 + 2,-3.4) {
    \begin{varwidth}{\linewidth}
       \[
            (\lambda, p_{2})
        \]
    \end{varwidth}
    };
    % Prosumer agent n
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (leftGeneration) at (4.05 + 3.5,-2.55) {complete \\ information of $P_{n}$};
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightGeneration) at (5.7 + 4,-3.4) {
    \begin{varwidth}{\linewidth}
       \[
            (\lambda, p_{n})
        \]
    \end{varwidth}
    };
    
\end{tikzpicture}
\end{figure*}

==> figures/src/coupling.tex <==
\section{Model coupling problem}

\begin{figure*}[h]
 % \centering
\begin{tikzpicture}[scale=0.99]
    % Draw model coupling main frame
    % \node[draw, rectangle, rounded corners, minimum width=11cm, minimum height=7.95cm, font=\scriptsize, dash pattern=on 5pt off 3pt] (mainrectframe) at (3.7,-0.61) {};

    % Draw the three rounded edge rectangles aligned at the top (Left)
    % ================================= Generator agent 1
    % ------------------------------------ Rounded end rectangle
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=1.2cm, align=center, font=\scriptsize] (leftrect1) at (-0.4,2.7) {Generator agent 1 \\ \\};
    % -------------------------------- Confidential bidding strategy rectangle
    \node[draw, rectangle, rounded corners, minimum width=2.6cm, minimum height=0.7cm, align=center, font=\tiny, fill=gray!60] (G1BiddingStrategy) at (-0.4,2.45) {Confidential \\ bidding strategy};
    % -------------------------------- Market schedule
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightHeatOperator) at (0.25, 1.8) {
    \begin{varwidth}{\linewidth}
       \[
            (\lambda, g_{1})
        \]
    \end{varwidth}
    };
    % =================================

    % ================================= Generator agent 2
    % ------------------------------------ Rounded end rectangle
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=1.2cm, align=center, font=\scriptsize] (leftrect2) at (3.5,2.7) {Generator agent 2 \\ \\};
    % -------------------------------- Confidential bidding strategy rectangle
    \node[draw, rectangle, rounded corners, minimum width=2.6cm, minimum height=0.7cm, align=center, font=\tiny, fill=gray!60] (G2BiddingStrategy) at (3.5,2.4) {Confidential \\ bidding strategy};
    % -------------------------------- Market schedule
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightEVOperator) at (2.65 + 1.5,1.8) {
    \begin{varwidth}{\linewidth}
       \[
             (\lambda, g_{2})
        \]
    \end{varwidth}
    };
    % =================================

    % ======================= invisible rectangle for the ... sign for generators 1 ... n
    \node[rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (lefttopinvisiblerect) at (5.7,2.6) {...};
    % =================================

    % ================================= Generator agent n
    % ------------------------------------ Rounded end rectangle
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=1.2cm, align=center, font=\scriptsize] (leftrect3) at (7.8,2.7) {Generator agent n \\ \\};
    % -------------------------------- Confidential bidding strategy rectangle
    \node[draw, rectangle, rounded corners, minimum width=2.6cm, minimum height=0.7cm, align=center, font=\tiny, fill=gray!60] (G2BiddingStrategy) at (7.8,2.4) {Confidential \\ bidding strategy};
    % -------------------------------- Market schedule
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightBEESOperator) at (5.45 + 3,1.8) {
    \begin{varwidth}{\linewidth}
       \[
            (\lambda, g_{n})
        \]
    \end{varwidth}
    };
    % =================================

    % ================================= Market operator ==================================
    % Draw a squared edge rectangle below the previous ones (Left)
    \node[draw, rectangle, minimum width=9cm, minimum height=2.7cm, align=center, font=\scriptsize] (leftmidrect) at (3.7, -0.6) {};

    \node[rectangle, minimum width=2cm, minimum height=1cm, align=center, font=\scriptsize] (marketoperatornamerect) at (3.8, 0.6) {Market operator agent};

    \node[rectangle, minimum width=5cm, minimum height=2.5cm, align=center, font=\scriptsize] (maxsocialwelfarerect) at (0.5 + 1.5, -0.6) {
        \\
        \begin{varwidth}{\linewidth}
            \[
                  \underset{g_{1} ... g_{n}, p_{1} ... p_{n}}\max  \text{Social welfare}
            \]
        \end{varwidth}
        \\
        \\
        \begin{varwidth}{\linewidth}
            \[
               \qquad  \qquad \text{s.t.} \sum^{N_{G}}_{i=1} {g_{i}} + \sum^{N_{P}}_{j=1} {p_{j}} = 0: \qquad  \qquad\lambda
            \]
        \end{varwidth} 
    };

    \node[rectangle, minimum width=2cm, minimum height=1cm, align=center, font=\tiny] (othermarketconsrect) at (0.7 + 1.5, -1.75) {\textit{Other market constraints}};
    % =========================================================================================

    % ========================== Merit order matching graph: by the market operator agent
   \node[rectangle, minimum width=2cm, minimum height=1cm, align=center, font=\tiny] (pricerect) at (2.8 + 2, 0.2) {Price};
    \node[rectangle, minimum width=2cm, minimum height=1cm, align=center, font=\tiny] (quantityrect) at (4.8 + 2, -1.87) {Quantity};
    \node[rectangle, minimum width=2cm, minimum height=1cm, align=center, font=\tiny] (Qrect) at (4.35 + 2, -1.6) {Q};

    \draw[->, line width=0.1mm] (3.2 + 2, -1.7) -- (5.15 + 2, -1.7) node[below] {};  % x-axis
    \draw[->, line width=0.1mm] (3.2 + 2, -1.7) -- (3.2 + 2, 0.3) node[left] {};  % y-axis
    
    \draw[line width=0.1mm] 
        (3.25 + 2, 0) -- (3.9 + 2, 0) -- (3.9 + 2, -0.3) -- (4.15 + 2, -0.3) 
        -- (4.15 + 2, -0.6) -- (4.5 + 2, -0.6) -- (4.5 + 2, -1.2) -- (4.75 + 2, -1.2)
        -- (4.75 + 2, -1.4) -- (4.9 + 2, -1.4) -- (4.9 + 2, -1.7);
    
    \draw[line width=0.1mm] 
        (3.25 + 2, -1.6) -- (3.95 + 2, -1.6) -- (3.95 + 2, -1.4) -- (4.25 + 2, -1.4) 
        -- (4.25 + 2, -1.2) -- (4.35 + 2, -1.2) -- (4.35 + 2, -1) -- (4.65 + 2, -1) -- (4.65 + 2, 0);
    
    \draw[dashed,line width=0.1mm] (3.0 + 2, -1) -- (4.35 + 2, -1);  % Horizontal dashed line
    \draw[dashed,line width=0.1mm] (4.5 + 2, -0.65) -- (4.5 + 2, -1.7);  % Vertical dashed line
    % ========================================================================================

    % ================================= Prosumer agent 1
    % ------------------------------------ Rounded end rectangle
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=1.2cm, align=center, font=\scriptsize] (leftrect4) at (-0.4, -3.9) {Prosumer agent 1 \\ \\};
    % -------------------------------- Confidential bidding strategy rectangle
    \node[draw, rectangle, rounded corners, minimum width=2.55cm, minimum height=0.7cm, align=center, font=\tiny, fill=gray!60] (P1BiddingStrategy) at (-0.4,-4.2) {Confidential \\ bidding strategy};
    % -------------------------------- Market schedule
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightElectrolyzer) at (0.25,-3) {
    \begin{varwidth}{\linewidth}
       \[
            (\lambda, p_{1})
        \]
    \end{varwidth}
    };
    % =================================

    % ================================= Prosumer agent 2
    % ------------------------------------ Rounded end rectangle
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=1.2cm, align=center, font=\scriptsize] (leftrect5) at (3.5, -3.9) {Prosumer agent 2 \\ \\};
    % -------------------------------- Confidential bidding strategy rectangle
    \node[draw, rectangle, rounded corners, minimum width=2.55cm, minimum height=0.7cm, align=center, font=\tiny, fill=gray!60] (P2BiddingStrategy) at (3.5,-4.2) {Confidential \\ bidding strategy};
    % -------------------------------- Market schedule
     \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightTradLoad) at (2.65 + 1.5,-3) {
    \begin{varwidth}{\linewidth}
       \[
            (\lambda, p_{2})
        \]
    \end{varwidth}
    };
    % =================================
    
    % ============== invisible rectangle for the ... sign for prosumers 1 ... n
    \node[rectangle, rounded corners, minimum width=0.5cm, minimum height=0.8cm, align=center, font=\scriptsize] (leftbottominvisiblerect) at (5.7,-4) {...};
    % ======================================================================

    % ================================= Prosumer agent n
    % ------------------------------------ Rounded end rectangle
    \node[draw, rectangle, rounded corners, minimum width=0.5cm, minimum height=1.2cm, align=center, font=\scriptsize] (leftrect6) at (7.8, -3.9) {Prosumer agent n \\ \\};
    % -------------------------------- Confidential bidding strategy rectangle
    \node[draw, rectangle, rounded corners, minimum width=2.55cm, minimum height=0.7cm, align=center, font=\tiny, fill=gray!60] (PnBiddingStrategy) at (7.8,-4.2) {Confidential \\ bidding strategy};
    % -------------------------------- Market schedule
    \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize] (rightGeneration) at (5.45 + 3,-3) {
    \begin{varwidth}{\linewidth}
       \[
            (\lambda, p_{n})
        \]
    \end{varwidth}
    };
    % =================================

    % ======================= Supply bid functions of Generator agents
    % ------------------------- Generator agent 1
    \draw[->, line width=0.1mm] (-1.5, 1.1) -- (-0.6, 1.1) node[below] {};  % x-axis
    \draw[->, line width=0.1mm] (-1.5, 1.1) -- (-1.5, 1.8) node[left] {};  % y-axis

    \draw[line width=0.1mm] 
        (-1.45, 1.15) -- (-1.2, 1.15) -- (-1.2, 1.4) -- (-1.05, 1.4) 
        -- (-1.05, 1.65) -- (-0.7, 1.65);

    % ------------------------- Generator agent 2
    \draw[->, line width=0.1mm] (2.4, 1.1) -- (3.3, 1.1) node[below] {};  % x-axis
    \draw[->, line width=0.1mm] (2.4, 1.1) -- (2.4, 1.8) node[left] {};  % y-axis

    \draw[line width=0.1mm] 
        (0.95 + 1.5, 1.15) -- (1.2 + 1.5, 1.15) -- (1.2 + 1.5, 1.4) -- (1.45 + 1.5, 1.4) 
    -- (1.45 + 1.5, 1.65) -- (1.7 + 1.5, 1.65);

    % ------------------------- Generator agent n
    \draw[->, line width=0.1mm] (6.7, 1.1) -- (7.6, 1.1) node[below] {};  % x-axis
    \draw[->, line width=0.1mm] (6.7, 1.1) -- (6.7, 1.8) node[left] {};  % y-axis
    
    \draw[line width=0.1mm] 
    (3.75 + 3, 1.15) -- (4.0 + 3, 1.15) -- (4.0 + 3, 1.4) -- (4.15 + 3, 1.4) 
    -- (4.15 + 3, 1.65) -- (4.5 + 3, 1.65);
    % =================================

    % ======================= Demand bid functions of Prosumer agents
    % ------------------------- Prosumer agent 1
    \draw[->, line width=0.1mm] (-1.5, -3.0) -- (-0.6, -3.0) node[below] {};  % x-axis
    \draw[->, line width=0.1mm] (-1.5, -3.0) -- (-1.5, -2.2) node[left] {};  % y-axis
    
    \draw[line width=0.1mm] (-1.45, -2.4) -- (-1.3, -2.4) -- (-1.3, -2.6) -- (-1.1, -2.6) 
        -- (-1.1, -2.78) -- (-0.8, -2.78) -- (-0.8, -3.0) -- (-0.8, -3.0);

    % ------------------------- Prosumer agent 2
    \draw[->, line width=0.1mm] (0.9 + 1.5, -3.0) -- (1.8 + 1.5, -3.0) node[below] {};  % x-axis
    \draw[->, line width=0.1mm] (0.9 + 1.5, -3.0) -- (0.9 + 1.5, -2.2) node[left] {};  % y-axis
    
   \draw[line width=0.1mm] (0.9 + 1.5, -2.9) -- (1.2 + 1.5, -2.9) -- (1.2 + 1.5, -2.6) -- (1.5 + 1.5, -2.6) -- (1.5 + 1.5, -2.3) -- (1.7 + 1.5, -2.3);

    % ------------------------- Prosumer agent n
    \draw[->, line width=0.1mm] (3.7 + 3, -3.0) -- (4.6 + 3, -3.0) node[below] {};  % x-axis
    \draw[->, line width=0.1mm] (3.7 + 3, -3.0) -- (3.7 + 3, -2.2) node[left] {};  % y-axis
    
    \draw[line width=0.1mm] (3.75 + 3, -2.4) -- (3.9 + 3, -2.4) -- (3.9 + 3, -2.6) -- (4.1 + 3, -2.6) 
    -- (4.1 + 3, -2.78) -- (4.4 + 3, -2.78) -- (4.4 + 3, -3.0) -- (4.4 + 3, -3.0);
    % =========================================================================

    % Arrows connecting rounded edge rectangles (left) to the left middle rectangle (leftmidrect)

    % Arrows connecting top rectangles (left) to leftmidrect
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect1.south) -- ++(0, -0.3) -- ([xshift=-0.1cm]leftmidrect.north -| leftrect1.south);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect1.south) -- ++(0, -0.3) -- ([xshift=0.1cm] leftmidrect.north -| leftrect1.south);
    
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect2.south) -- ++(0, -0.3) -- ([xshift=-0.1cm] leftmidrect.north -| leftrect2.south);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect2.south) -- ++(0, -0.3) -- ([xshift=0.1cm] leftmidrect.north -| leftrect2.south);
    
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect3.south) -- ++(0, -0.3) -- ([xshift=-0.1cm] leftmidrect.north -| leftrect3.south);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect3.south) -- ++(0, -0.3) -- ([xshift=0.1cm] leftmidrect.north -| leftrect3.south);

    
    % Arrows connecting bottom rectangles (left) to leftmidrect
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect4.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] leftmidrect.south -| leftrect4.north);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect4.north) -- ++(0, 0.3) -- ([xshift=0.1cm] leftmidrect.south -| leftrect4.north);
    
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect5.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] leftmidrect.south -| leftrect5.north);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect5.north) -- ++(0, 0.3) -- ([xshift=0.1cm] leftmidrect.south -| leftrect5.north);
    
    \draw[->, >=latex, line width=0.1mm] ([xshift=-0.1cm] leftrect6.north) -- ++(0, 0.3) -- ([xshift=-0.1cm] leftmidrect.south -| leftrect6.north);
    \draw[<-, >=latex, line width=0.1mm] ([xshift=0.1cm] leftrect6.north) -- ++(0, 0.3) -- ([xshift=0.1cm] leftmidrect.south -| leftrect6.north);

\end{tikzpicture}
\end{figure*}


==> figures/src/equilibrium.tex <==
\section{Equilibirum problem}

\begin{figure*}[h] % Non-cooperative Nash game
\begin{tikzpicture}[scale=0.95]

     \node[draw, rectangle, rounded corners, minimum width=9.2cm, minimum height=5.8cm, font=\scriptsize, dash pattern=on 5pt off 3pt] (mainrectframe) at (2.7,1.75) {};

    % \node[rectangle, rounded corners, minimum width=12cm, minimum height=1cm, font=\scriptsize] (invisiblerecttop) at (3,4.8) {Equilibrium problem};

    % \path[draw, line width=0.05mm, name path=linewithconstraintatbottom, dash pattern=on 3pt off 2pt] (-2.1, 0.01) -- (7.5, 0.01);
    
     \node[rectangle, rounded corners, minimum width=8cm, minimum height=1cm, font=\scriptsize] (invisiblerectbottom) at (2.7,-0.55) {s.t. \quad Linking constraint: \\
        \\  
        \begin{varwidth}{\linewidth}
            \[
               \quad \sum^{N_{G}}_{i=1} {g^{k}_{i}} + \sum^{N_{P}}_{j=1} {p^{k}_{j}} = 0: \quad \quad \lambda
            \]
        \end{varwidth}
     };
     
    % Draw the three rounded edge rectangles aligned at the top (Left)
    \node[draw, rectangle, rounded corners, minimum width=2.4cm, minimum height=1.8cm, align=center, font=\scriptsize] (leftrect1) at (-0.6,3.5) {Generator agent 1 \\
        \\
        \begin{varwidth}{\linewidth}
        \[
            \textstyle  \underset{g_{1}}\max \prod \big( \displaystyle g_{1},  \chi_{-1}, \lambda \big)
        \]
        \end{varwidth}
        \\
        \begin{varwidth}{\linewidth}
        \[
             \text{s.t.} \quad g_{1} \in G_{1}
        \]
        \end{varwidth}
    };
    
    \node[draw, rectangle, rounded corners, minimum width=2.4cm, minimum height=1.8cm, align=center, font=\scriptsize] (leftrect1) at (2.4,3.5) {Generator agent 2 \\
        \\
        \begin{varwidth}{\linewidth}
        \[
            \textstyle \underset{g_{2}}\max \prod \big( \displaystyle g_{2},  \chi_{-1}, \lambda \big)
        \]
        \end{varwidth}
        \\
        \begin{varwidth}{\linewidth}
        \[
             \text{s.t.} \quad g_{2} \in G_{2}
        \]
        \end{varwidth}
    };
    
    % invisible rectangle for the ... sign for generators 1 ... n
    \node[rectangle, rounded corners, minimum width=2.4cm, minimum height=1.8cm, align=center, font=\scriptsize] (lefttopinvisiblerect) at (4.2,2.35) {\textbf{...}};

    \node[draw, rectangle, rounded corners, minimum width=2.4cm, minimum height=1.8cm, align=center, font=\scriptsize] (leftrect1) at (6,3.5) {Generator agent n \\
        \\
        \begin{varwidth}{\linewidth}
        \[
            \textstyle \underset{g_{n}}\max \prod \big( \displaystyle g_{n},  \chi_{-1}, \lambda \big)
        \]
        \end{varwidth}
        \\
        \begin{varwidth}{\linewidth}
        \[
             \text{s.t.} \quad g_{n} \in G_{n}
        \]
        \end{varwidth}
    };
    
    %  % Draw three rounded edge rectangles aligned at the bottom (Left)
    \node[draw, rectangle, rounded corners,minimum width=2.4cm, minimum height=1.8cm, align=center, font=\scriptsize] (leftrect1) at (-0.6,1.2) {Prosumer agent 1 \\
        \\
        \begin{varwidth}{\linewidth}
        \[
            \textstyle \underset{p_{1}}\max \prod \big( \displaystyle p_{1},  \chi_{-1}, \lambda \big)
        \]
        \end{varwidth}
        \\
        \begin{varwidth}{\linewidth}
        \[
             \text{s.t.} \quad p_{1} \in P_{1}
        \]
        \end{varwidth}
    };
    
     \node[draw, rectangle, rounded corners, minimum width=2.4cm, minimum height=1.8cm, align=center, font=\scriptsize] (leftrect1) at (2.4,1.2) {Prosumer agent 2 \\
        \\
        \begin{varwidth}{\linewidth}
        \[
            \textstyle \underset{p_{2}}\max \prod \big( \displaystyle p_{2},  \chi_{-1}, \lambda \big)
        \]
        \end{varwidth}
        \\
        \begin{varwidth}{\linewidth}
        \[
             \text{s.t.} \quad p_{2} \in P_{2}
        \]
        \end{varwidth}
    };
    
    \node[draw, rectangle, rounded corners, minimum width=2.4cm, minimum height=1.8cm, align=center, font=\scriptsize] (leftrect1) at (6,1.2) {Prosumer agent n \\
        \\
        \begin{varwidth}{\linewidth}
        \[
            \textstyle \underset{p_{n}}\max \prod \big( \displaystyle p_{n},  \chi_{-1}, \lambda \big)
        \]
        \end{varwidth}
        \\
        \begin{varwidth}{\linewidth}
        \[
             \text{s.t.} \quad p_{n} \in P_{n}
        \]
        \end{varwidth}
    };
    
\end{tikzpicture}
\end{figure*}

==> figures/src/time_space.tex <==
\section{Time-space plot for varying problem size}

\begin{figure*}[h] % ADMM-model interactions
    \begin{tikzpicture}[scale=0.95]
        %  ========================== Space (number of agents)
        \draw[->, line width=0.1mm] (10, 0) -- (15.5, 0) node[below] {};  % x-axis

        \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, above] (space) at (15.5, -1.3) {Space (number of agents)};

        \draw[-, >=latex, line width=0.1mm] (10.5, -0.1) -- (10.5, 0.1); % 5
        \node at (10.5, -0.3) {\scriptsize 5};
        
        \draw[-, >=latex, line width=0.1mm] (11, -0.1) -- (11, 0.1); % 10
        \node at (11, -0.3) {\scriptsize 10};
        
        \draw[-, >=latex, line width=0.1mm] (11.6, -0.1) -- (11.6, 0.1); % 25
        \node at (11.6, -0.3) {\scriptsize 25};
        
        \draw[-, >=latex, line width=0.1mm] (12.4, -0.1) -- (12.4, 0.1); % 50
        \node at (12.4, -0.3) {\scriptsize 50};
        
        \draw[-, >=latex, line width=0.1mm] (13.4, -0.1) -- (13.4, 0.1); % 100
        \node at (13.4, -0.3) {\scriptsize 100};
        
        \draw[-, >=latex, line width=0.1mm] (14.6, -0.1) -- (14.6, 0.1); % 250
        \node at (14.6, -0.3) {\scriptsize 250};

         %  ========================== Time (horizon)
        \draw[->, line width=0.1mm] (10, 0) -- (10, 4) node[left] {};  % y-axis
    
        \node[rectangle, minimum width=1cm, minimum height=1cm, align=center, font=\scriptsize, rotate=90, above] (space) at (9.5, 3.7) {Time \\ (horizon)};
    
        \draw[-, >=latex, line width=0.1mm] (9.9, 0.3) -- (10.1, 0.3); % 24h
        \node at (9.6, 0.3) {\scriptsize 24h};
        
        \draw[-, >=latex, line width=0.1mm] (9.9, 0.7) -- (10.1, 0.7); % 7d
        \node at (9.6, 0.7) {\scriptsize 7d};
        
        \draw[-, >=latex, line width=0.1mm] (9.9, 1.2) -- (10.1, 1.2); % 1m
        \node at (9.6, 1.2) {\scriptsize 1m};
        
        \draw[-, >=latex, line width=0.1mm] (9.9, 1.8) -- (10.1, 1.8); % 6m
        \node at (9.6, 1.8) {\scriptsize 6m};
        
        \draw[-, >=latex, line width=0.1mm] (9.9, 2.5) -- (10.1, 2.5); % 1y
        \node at (9.6, 2.5) {\scriptsize 1y};
        
        \draw[-, >=latex, line width=0.1mm] (9.9, 3.5) -- (10.1, 3.5); % 5y
        \node at (9.6, 3.5) {\scriptsize 5y};

        % Draw (plot) points for all combinations
        \filldraw (10.5, 0.3) circle (2pt);  % (5 agents, 24h)
        \filldraw (10.5, 0.7) circle (2pt);  % (5 agents, 7d)
        \filldraw (10.5, 1.2) circle (2pt);  % (5 agents, 1m)
        \filldraw (10.5, 1.8) circle (2pt);  % (5 agents, 6m)
        \filldraw (10.5, 2.5) circle (2pt);  % (5 agents, 1y)
        \filldraw (10.5, 3.5) circle (2pt);  % (5 agents, 5y)

        \filldraw (11, 0.3) circle (2pt);    % (10 agents, 24h)
        \filldraw (11, 0.7) circle (2pt);    % (10 agents, 7d)
        \filldraw (11, 1.2) circle (2pt);    % (10 agents, 1m)
        \filldraw (11, 1.8) circle (2pt);    % (10 agents, 6m)
        \filldraw (11, 2.5) circle (2pt);    % (10 agents, 1y)
        \filldraw (11, 3.5) circle (2pt);    % (10 agents, 5y)

        \filldraw (11.6, 0.3) circle (2pt);  % (25 agents, 24h)
        \filldraw (11.6, 0.7) circle (2pt);  % (25 agents, 7d)
        \filldraw (11.6, 1.2) circle (2pt);  % (25 agents, 1m)
        \filldraw (11.6, 1.8) circle (2pt);  % (25 agents, 6m)
        \filldraw (11.6, 2.5) circle (2pt);  % (25 agents, 1y)
        \filldraw (11.6, 3.5) circle (2pt);  % (25 agents, 5y)

        \filldraw (12.4, 0.3) circle (2pt);  % (50 agents, 24h)
        \filldraw (12.4, 0.7) circle (2pt);  % (50 agents, 7d)
        \filldraw (12.4, 1.2) circle (2pt);  % (50 agents, 1m)
        \filldraw (12.4, 1.8) circle (2pt);  % (50 agents, 6m)
        \filldraw (12.4, 2.5) circle (2pt);  % (50 agents, 1y)
        \filldraw (12.4, 3.5) circle (2pt);  % (50 agents, 5y)

        \filldraw (13.4, 0.3) circle (2pt);  % (100 agents, 24h)
        \filldraw (13.4, 0.7) circle (2pt);  % (100 agents, 7d)
        \filldraw (13.4, 1.2) circle (2pt);  % (100 agents, 1m)
        \filldraw (13.4, 1.8) circle (2pt);  % (100 agents, 6m)
        \filldraw (13.4, 2.5) circle (2pt);  % (100 agents, 1y)
        \filldraw (13.4, 3.5) circle (2pt);  % (100 agents, 5y)

        \filldraw (14.6, 0.3) circle (2pt);  % (250 agents, 24h)
        \filldraw (14.6, 0.7) circle (2pt);  % (250 agents, 7d)
        \filldraw (14.6, 1.2) circle (2pt);  % (250 agents, 1m)
        \filldraw (14.6, 1.8) circle (2pt);  % (250 agents, 6m)
        \filldraw (14.6, 2.5) circle (2pt);  % (250 agents, 1y)
        \filldraw (14.6, 3.5) circle (2pt);  % (250 agents, 5y)
         
    \end{tikzpicture}
\end{figure*}

==> storyline.tex <==
1. Motivation: Coordination challenge in MIES

Goal: establish the real-world problem.

Content:

Increasing penetration of flexible energy resources

Flexibility provided by heterogeneous, autonomous agents

Need to coordinate flexibility across multiple energy carriers (electricity, heat, gas)

Key message:

Modeling the coordination of flexibility scheduling among many autonomous agents is a central challenge in MIES.

2. Conventional modeling approach

Goal: establish the baseline used in literature.

Content:

Most studies model flexibility coordination using co-optimization

A single global optimization problem

Central operator determines dispatch decisions

Key message:

This corresponds to centralized coordination implemented through monolithic optimization.

3. Limitations of centralized monolithic models

Goal: motivate alternative representations.

Main issues:

Lack of autonomy

Privacy concerns

Poor scalability

Key message:

These assumptions conflict with the operational reality of decentralized flexibility providers.

4. Alternative modeling paradigm introduced in this work

Goal: introduce model coupling as your conceptual framework.

Content:

Instead of a monolithic model, represent each agent with its own model

Coordination occurs through exchange of interface variables

This modeling paradigm is known as model coupling

Key message:

Model coupling allows representing autonomous agents while coordinating their interactions.

Important:
You are not claiming literature already does this extensively — you are introducing it as a framework to study coordination architectures.

5. Coordination architectures under model coupling

Goal: introduce the key conceptual idea of the paper.

Within the model coupling paradigm, two coordination architectures can be implemented:

Distributed coordination

agents cooperate to optimize a shared objective

implemented through iterative price-response

Decentralized coordination

agents interact through market mechanisms

coordination through auction-based clearing

Key message:

Model coupling enables both distributed and decentralized coordination architectures.

6. Gap in the literature

Goal: position your contribution.

Content:

Most studies focus on centralized co-optimization

Limited work studying coordination architectures among autonomous agents

No systematic comparison between these coordination approaches

Key message:

The trade-offs between centralized, distributed, and decentralized coordination remain poorly understood.

7. Paper contribution

Goal: state clearly what the paper does.

This paper:

Introduces a taxonomy of coordination approaches for flexibility scheduling

Formalizes three coordination models

centralized co-optimization

distributed price-response model coupling

decentralized market-auction model coupling

Implements them as open-source frameworks

Benchmarks optimality, autonomy, and scalability trade-offs

Reference Table 1.

8. Paper structure

Standard closing paragraph.

The one-sentence storyline

Your introduction should read conceptually like this:

While flexibility scheduling in multi-energy systems is typically modeled using centralized co-optimization, this approach poorly represents the autonomy and privacy of real-world flexibility providers. To address this, we introduce a model coupling paradigm in which autonomous subsystem models interact through defined interfaces. Within this paradigm, we study two coordination architectures—distributed price-response coordination and decentralized market-auction coordination—and compare them with centralized co-optimization.

Why this framing is strong

This positioning makes your paper about:

A taxonomy and comparison of coordination architectures for MIES.

Not just:

"Here is a new market mechanism."

That makes the work much more scientific and generalizable.



% ==============================================
Within the model coupling paradigm, the coordination of interactions among agents can be implemented under different coordination architectures. In this work, we consider two fundamentally different approaches: a price-response–based approach that follows a distributed coordination architecture, and a market auction–based approach that follows a decentralized coordination architecture.

In the price-response approach, agents locally optimize their dispatch decisions and interact to cooperatively optimize a global utility. The required information exchange includes: (1) point-wise demand–supply time series computed locally by each agent as a response to prices broadcast by a coordinating entity; and (2) the system imbalance, defined as the difference between total demand and supply. Since agents’ dispatch decisions are coupled through the system-wide power balance constraint, prices and dispatch decisions are iteratively updated based on this imbalance until a consensus price is reached at which the imbalance is below a specified threshold. Provided an equilibrium exists, such iterative procedures can converge to a solution that is close to that of co-optimization. However, this approach also has several limitations. First, the autonomy of agents is partial, as their local decisions are influenced over iterations to align with a global objective. Second, the iterative nature of the coordination process can lead to high computational costs, since decisions are recomputed over the full simulation horizon at each iteration. As a result, the approach can scale poorly for large-scale systems with long time horizons. Moreover, convergence is not guaranteed in general, particularly in the presence of non-convexities such as integer decision variables.

Alternatively, coordination can be implemented using a market auction–based approach that follows a decentralized architecture. In this case, agents retain full autonomy over their local dispatch decisions and interact by submitting demand and supply bid functions that internalize their techno-economic and intertemporal constraints. These bids are then matched through a market-clearing mechanism that maximizes social welfare over a given time window. Compared to the price-response approach, this mechanism shifts coordination from an iterative process to a sequence of market-clearing problems, typically solved over a rolling horizon. This can offer advantages in terms of scalability, as the full time horizon is decomposed into smaller subproblems. In addition, since only bid functions are exchanged, agents can preserve the privacy of their internal models. However, this decentralized coordination may lead to solutions that deviate from the global optimum achieved by co-optimization or its distributed counterpart, reflecting a trade-off between optimality and scalability.

In summary, the model coupling paradigm enables multiple coordination approaches that differ fundamentally in how agents interact and how system-wide consistency is enforced. Distributed price-response approaches can approximate globally optimal solutions but may face challenges in terms of computational efficiency and convergence. Decentralized market-based approaches, on the other hand, offer improved scalability and stronger autonomy and privacy guarantees, but may sacrifice optimality. A summary of these differences is provided in Table~\ref{tab:table1}, highlighting the trade-offs between coordination architecture, information exchange, autonomy, optimality, and scalability.
